Pseudonymization at Scale: OLCF's Summit Usage Data Case Study

The analysis of vast amounts of data and the processing of complex computational jobs have traditionally relied upon high performance computing (HPC) systems. Understanding these analyses' needs is paramount for designing solutions that can lead to better science, and similarly, understanding the characteristics of the user behavior on those systems is important for improving user experiences on HPC systems. A common approach to gathering data about user behavior is to analyze system log data available only to system administrators. Recently at Oak Ridge Leadership Computing Facility (OLCF), however, we unveiled user behavior about the Summit supercomputer by collecting data from a user's point of view with ordinary Unix commands. Here, we discuss the process, challenges, and lessons learned while preparing this dataset for publication and submission to an open data challenge. The original dataset contains personal identifiable information (PII) about OLCF users which needed be masked prior to publication, and we determined that anonymization, which scrubs PII completely, destroyed too much of the structure of the data to be interesting for the data challenge. We instead chose to pseudonymize the dataset to reduce its linkability to users' identities. Pseudonymization is significantly more computationally expensive than anonymization, and the size of our dataset, approximately 175 million lines of raw text, necessitated the development of a parallelized workflow that could be reused on different HPC machines. We demonstrate the scaling behavior of the workflow on two leadership class HPC systems at OLCF, and we show that we were able to bring the overall makespan time from an impractical 20+ hours on a single node down to around 2 hours. As a result of this work, we release the entire pseudonymized dataset and make the workflows and source code publicly available.

==> sec-impl.tex <==
\section{Implementation}
\label{sec:impl}

As part of this paper, we release the complete code publicly and encourage the community to reuse it as an efficient and parallelized data pseudonymization. The code may be adapted to varied needs such as anonymization, reverse-pseudonymization and may be repurposed as a scalable data processing pipeline.

The Github URL for the code involved is~\cite{Maheshwari_loginanalysis_2022}.
 organization .. explanation ..

This is the first Swift/T implementation of a workflow on Summit as far as we know.


==> sec-results.tex <==
\section{Results}
\label{sec:results}

% About crusher
% Crusher is a National Center for Computational Sciences (NCCS) moderate-security system that contains identical hardware and similar software as the upcoming Frontier system~\cite{crusher}. It is used as an early-access testbed for Center for Accelerated Application Readiness (CAAR) and Exascale Computing Project (ECP) teams as well as NCCS staff and the vendor partners. The system has 2 cabinets, the first with 128 compute nodes and the second with 64 compute nodes, for a total of 192 compute nodes.


Strong and Weak Scaling results. Ability to apply this workflow in production. Running at scale on Summit. Release the resulting dataset.

We suspect the performance variability is correlated with the performance of
the GPFS File system. So, we study the times of our scalability runs and how 
was GPFS performance during those times using our collected data.




